Enhancing the Privacy of Federated Learning with Sketching

In response to growing concerns about user privacy, federated learning has emerged as a promising tool to train statistical models over networks of devices while keeping data localized. Federated learning methods run training tasks directly on user devices and do not share the raw user data with third parties. However, current methods still share model updates, which may contain private information (e.g., one's weight and height), during the training process. Existing efforts that aim to improve the privacy of federated learning make compromises in one or more of the following key areas: performance (particularly communication cost), accuracy, or privacy. To better optimize these trade-offs, we propose that \textit{sketching algorithms} have a unique advantage in that they can provide both privacy and performance benefits while maintaining accuracy. We evaluate the feasibility of sketching-based federated learning with a prototype on three representative learning models. Our initial findings show that it is possible to provide strong privacy guarantees for federated learning without sacrificing performance or accuracy. Our work highlights that there exists a fundamental connection between privacy and communication in distributed settings, and suggests important open problems surrounding the theoretical understanding, methodology, and system design of practical, private federated learning.

==> sections/related.tex <==
\section{Related Work}

\gs{Given the space limitations, I wonder if this section is necessary? It seems like you've done a nice job in covering the related work already in the intro and background sections.}
\tian{agree}

\para{Sketching in network measurement.} Sketches are designed for many measurement tasks such as: 
(1) Heavy hitter detection to identify large flows, such as~\cite{CMSketch,SpaceSavings,CountSketch,univmon,HashPipe}.
(2) Change detection to identify flows that change significantly over two consecutive time intervals(e.g.,~\cite{k-ary,revsketch,univmon}). (3) Entropy estimation to approximate the entropy of different network workload (e.g.,~\cite{Lall:2006,univmon}).


% sketch (+privacy, +communication reduction)
\para{Sketching in other machine learning setting.} Recent work~\cite{acharya2019distributed,jiang2018sketchml,ivkin2019communication} explores the feasibility of leveraging sketches to reduce the overall communication cost in a general distributed machine learning setting. An idea of leveraging sketches in their setting is to preserve the identities of significant model updates and only send the model updates containing the significant coordinates.

\para{Privacy mechanism for federated learning.}
